Discrete Price Updates Yield Fast Convergence in Ongoing Markets with Finite Warehouses

This paper shows that in suitable markets, even with out-of-equilibrium trade allowed, a simple price update rule leads to rapid convergence toward the equilibrium. In particular, this paper considers a Fisher market repeated over an unbounded number of time steps, with the addition of finite sized warehouses to enable non-equilibrium trade. The main result is that suitable tatonnement style price updates lead to convergence in a significant subset of markets satisfying the Weak Gross Substitutes property. Throughout this process the warehouse are always able to store or meet demand imbalances (the needed capacity depends on the initial imbalances). Finally, our price update rule is robust in a variety of regards: 1. The updates for each good depend only on information about that good (its current price, its excess demand since its last update) and occur asynchronously from updates to other prices. 2. The process is resilient to error in the excess demand data. 3. Likewise, the process is resilient to discreteness, i.e. a limit to divisibility, both of goods and money.

==> mut-d-simple.tex <==
\subsection{Multiple Goods, Bounded Demand}

Suppose that there are $n$ goods $g_1, g_2,  \cdots , g_n )$. 
Let $p= (p_1 ,p_2 , \cdots,p_n)$ be the $n$-vector of prices
for these goods, 
and let  $x_i(p)$, or  $x_i$ for short, 
denote the demand for the $i$th good at prices $p$ 
(that is, it is a function of all the prices, 
not just the price of the $i$th good). 
Again, we assume that

Again, we use the update rule
\[
\label{eqn:p-update-i}
p_i'=p_i \left(1+ \lmbd \min\left\{ 1, \frac{x_i-w_i}{w_i} \right\} \right)
\]
Again, we assume that the demands satisfy
\[
\frac{x_i(p)}{p_i} \le -\frac{dx_i}{dp_i} \le E\frac{x_i(p)}{p_i},
       ~~\mbox{where } 1\le E\le \frac{1}{2\lambda}.
\]
%

We use the potential function $\phi = \sum_i \phi_i $, 
where $\phi_i = p _i |x _i - w _i| $.
So the effect of an update to $p_i$ on $\phi_i$ is just as in the 1-D case. 
However it may affect the demands $x_j$ 
and hence $\phi _j$ for goods $j \ne i$. 
Before we quantify this we introduce some more notation. 
Let $I$ denote $\phi_i(p) \min\{ 1 , \frac{w _i}{x_i - w_i} \} $.
Let $p_{- i }, p'_ i $ denote the price vector $ p $ 
with the $i$th price replaced by $p'_ i $. 
Let $| \Delta  \phi _ j =  \phi _ j ( p _{- i }, p'_ i ) - \phi_ j ( p _{- i }, p _ i ) $ 
for all $j$.

To achieve a similar rate of progress as in the 1-D case
we assume that the following property holds.

\begin{property}
\[
| \Delta  \phi _ j  | + \alpha  I  \le  \Delta   \phi _ i
\]
\end{property}

The term on the RHS is the reduction in $\phi_i$. 
The sum on the LHS represents the change to the $\phi_j $, 
$j \ne i$, which are assumed, in a worst-case way, 
to all be increases (which is possible with certain $w_j$, 
namely  $w_j > x_j > x'_j $  or $w_j < x_j < x'_j $). 
